Generating Tips from Song Reviews: A New Dataset and Framework

Reviews of songs play an important role in online music service platforms. Prior research shows that users can make quicker and more informed decisions when presented with meaningful song reviews. However, reviews of music songs are generally long in length and most of them are non-informative for users. It is difficult for users to efficiently grasp meaningful messages for making decisions. To solve this problem, one practical strategy is to provide tips, i.e., short, concise, empathetic, and self-contained descriptions about songs. Tips are produced from song reviews and should express non-trivial insights about the songs. To the best of our knowledge, no prior studies have explored the tip generation task in music domain. In this paper, we create a dataset named MTips for the task and propose a framework named GENTMS for automatically generating tips from song reviews. The dataset involves 8,003 Chinese tips/non-tips from 128 songs which are distributed in five different song genres. Experimental results show that GENTMS achieves top-10 precision at 85.56%, outperforming the baseline models by at least 3.34%. Besides, to simulate the practical usage of our proposed framework, we also experiment with previously-unseen songs, during which GENTMS also achieves the best performance with top-10 precision at 78.89% on average. The results demonstrate the effectiveness of the proposed framework in tip generation of the music domain.

==> sections/liter.tex <==
\section{Related work}
\label{sec:Related Work}
\subsection{Music Review Mining}
Mining music reviews has long been studied. Hu et al.~\cite{DBLP:conf/ismir/HuDWE05} demonstrate a system to predict star rating assigned to the music by classifying reviews according to the genre of the music. In fact, in addition to star rating, we can also assign text messages to music, which is more acceptable to users. 
Printer et al.~\cite{DBLP:conf/icwsm/PinterPSB20} create a dataset of expert reviews and offeHr several possible avenues for research. Different from their study in expert reviews, most of the work still focus on analyzing user reviews. Oramas et al.~\cite{DBLP:conf/ismir/OramasALSS16} explore a multimodal dataset constructed from albums and Amazon customer reviews. They analyze the potential correlation between sentiment and key culture events in music reviews.
Although prior researches have found music reviews useful for attracting potential users, 
no one studies the use of short sentences for the music songs, which is also known as ``Tips'' in the product domain~\cite{DBLP:conf/wsdm/HirschNGN21}. Previous studies show that ``Tips'' in the product domain is beneficial for item recommendation~\cite{DBLP:conf/cikm/YangHLWWZFHZW20}.

\subsection{Tip Generation in Product Domain}
Customer reviews contain valuable information which is useful for making a purchase decision. 
To help customers extract this information, researchers suggest new tasks of generating representative sentences from reviews for a given product. 
Gamzu et al.~\cite{DBLP:conf/naacl/GamzuGKLA21} propose an identification task on ``helpful sentence'' that is defined as individual sentence and can be helpful and faithful in a purchase decision.
Hirsch et al.~\cite{DBLP:conf/wsdm/HirschNGN21} define a tip in product domain as a short, concise, practical, and self-contained piece of advice, and publish an English dataset.
Several methods have been proposed for generating tips from user reviews.
For example, based on Transformer~\cite{vaswani2017attention}, Yang et al.~\cite{DBLP:conf/cikm/YangHLWWZFHZW20} propose a query-aware tip generation model for a popular e-commerce application, Dianping, but the dataset is not publicly available. 
Li et al.~\cite{DBLP:conf/www/LiWBL19, DBLP:conf/sigir/LiWRBL17} explore abstractive tip generation. 
However, they just enrich the representation of users and items with reviews in the training stage and do not introduce reviews to operating stage.
In this paper, we do not consider specific users but only focus on extracting representative tips to for a song.

\subsection{Text Summarization}
Text summarization is relevant to the tip generation,
% Closest to the tip generation task is text summarization, 
which has been studied for a long time and is valuable to our task. 
Text summarization seeks to generate several sentences as a summary, which focuses on balancing the salience and redundancy of sentences. 
TextRank~\cite{DBLP:conf/emnlp/MihalceaT04} focuses on homogeneous graphs constructed with the content similarity among sentences. 
The heterogeneous graph shows its superiority by leveraging words as intermediate nodes~\cite{DBLP:conf/acl/WangLZQH20}.
Most of recent text summarization methods like BertSum~\cite{DBLP:conf/emnlp/LiuL19} encode the entire article, which is suitable for single-document-level summarization.
However, our task is to extract sentences from multiple reviews of a song, which is more similar to MDS (Multi-document Summarization) and the quantity of documents is not small.
Ma et al.~\cite{DBLP:journals/corr/abs-2011-04843} survey the deep learning techniques in MDS. The method of concatenation for multiple documents is still a research focus. 
Above methods focus on the salience of sentences and do not consider the redundancy. 
To mitigate the redundancy between extracted sentences, Zhou et al.~\cite{DBLP:conf/coling/ZhouWZ20} extract sub-sentential units based on the constituency parsing tree to construct a summary. 
Wu et al.~\cite{DBLP:conf/coling/YuanWL20} apply dependency analysis to sentences and propose an empirical method to split sentences into smaller units called ``fact''. However, these small units~\cite{DBLP:conf/acl/XuGCL20} decrease the readability of summary which is unacceptable in our task. 
Cho et al.~\cite{DBLP:conf/acl/ChoLFL19} present a novel method inspired by DPP (Determinantal Point Process)~\cite{DBLP:journals/ftml/KuleszaT12} and capsule network to improve the similarity measure in extractive multi-document summarization. 
The redundancy, in other words, diverse content is also important when generating multiple tips for a song. 
